Probing the Mid-level Vision Capabilities of Self-Supervised Learning

Mid-level vision capabilities - such as generic object localization and 3D geometric understanding - are not only fundamental to human vision but are also crucial for many real-world applications of computer vision. These abilities emerge with minimal supervision during the early stages of human visual development. Despite their significance, current self-supervised learning (SSL) approaches are primarily designed and evaluated for high-level recognition tasks, leaving their mid-level vision capabilities largely unexamined. In this study, we introduce a suite of benchmark protocols to systematically assess mid-level vision capabilities and present a comprehensive, controlled evaluation of 22 prominent SSL models across 8 mid-level vision tasks. Our experiments reveal a weak correlation between mid-level and high-level task performance. We also identify several SSL methods with highly imbalanced performance across mid-level and high-level capabilities, as well as some that excel in both. Additionally, we investigate key factors contributing to mid-level vision performance, such as pretraining objectives and network architectures. Our study provides a holistic and timely view of what SSL models have learned, complementing existing research that primarily focuses on high-level vision tasks. We hope our findings guide future SSL research to benchmark models not only on high-level vision tasks but on mid-level as well.

==> figs/best_performing.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figs/source/best_performing.pdf}
\vspace*{-10pt}
\caption{\textbf{Performance of Top SSL Models Across Mid-Level Vision Tasks.} This heatmap shows the relative performance of best-performing self-supervised learning (SSL) models on various mid-level vision tasks, highlighting each task's top model with a bold border. Each row is normalized to emphasize model strengths in tasks like segmentation, depth estimation, and surface normals.}
\label{fig:best_performing}
\end{figure}

==> figs/correspondence.tex <==
\begin{figure*}[htbp]
\centering
\begin{tabular}{cc}
    \includegraphics[width=\linewidth]{figs/source/correspondence.pdf}
\end{tabular}
\vspace*{-10pt}
\caption{\textbf{Mid-level Vision Tasks} We demonstrate each task of mid-level vision tasks with one example.}
\label{fig:depth_visualization}
\end{figure*}

==> figs/correspondence_visualization.tex <==
\begin{figure*}[ht!]
    \centering
    % \fbox{\rule{0pt}{100pt} \rule{400pt}{0pt}} \\
    \includegraphics[width=0.7\linewidth]{figs/source/correspondence_visualization.pdf}
    % \vspace{-6mm}
    \caption{\textbf{Qualitative Object Correspondence Visualizations for Selected SSL Models.} Geometry correspondence visualizations are shown for selected SSL models. Green indicates correct predicted correspondence and red means wrong predicted correspondence.}
\label{fig:qualitative-corr}
\end{figure*}

==> figs/depth_nyuv2_visualization.tex <==
\begin{figure*}[htbp]
\centering
\begin{tabular}{cc}
    \includegraphics[width=\linewidth]{figs/source/depth_NYUv2.jpg}
\end{tabular}
\vspace*{-10pt}
\caption{\textbf{Depth Visualization on NYUv2}}
\label{fig:depth_visualization}
\end{figure*}

==> figs/mae_ranking.tex <==
\begin{figure}[t]
    \centering
    % \fbox{\rule{0pt}{100pt} \rule{150pt}{0pt}} \\
    \includegraphics[width=\linewidth]{figs/source/mae_rank_across_tasks.pdf}
    % \vspace{-6mm}
    \caption{Evaluation of MAE model rankings across ImageNet Linear Probing and mid-level vision tasks relevant to object segmentation, depth, surface normals, reshading, and similarity. This analysis demonstrates MAE’s comparative strengths in different tasks, highlighting its versatility across high-level and mid-level visual representations. Lower bars signify higher performance ranking.}
    \label{fig:mae_ranking}
\end{figure}

==> figs/maskfeat_ranking.tex <==
\begin{figure}[t]
    \centering
    % \fbox{\rule{0pt}{100pt} \rule{150pt}{0pt}} \\
    \includegraphics[width=\linewidth]{figs/source/maskfeat_rank_across_tasks.pdf}
    % \vspace{-6mm}
    \caption{Evaluation of MaskFeat model rankings across ImageNet Linear Probing and mid-level vision tasks relevant to object segmentation, depth, surface normals, reshading, and similarity. This analysis demonstrates MaskFeat’s comparative strengths in different tasks, highlighting its versatility across high-level and mid-level visual representations. Lower bars signify higher performance ranking.}
    \label{fig:maskfeat_ranking}
\end{figure}

==> figs/mid-level-vision-demonstrations.tex <==
\begin{figure*}[htbp]
\centering
\begin{tabular}{cc}
    \includegraphics[width=\linewidth]{figs/source/mid-level-probing.pdf}
\end{tabular}
\vspace*{-10pt}
\caption{\textbf{Mid-level Vision Tasks} We demonstrate each task of mid-level vision tasks with one example. \zc{how about high-level vision vs mid-level vision tasks?}}
\label{fig:midvsin1k}
\end{figure*}

==> figs/qualitative.tex <==
\begin{figure*}[t]
    \centering
    \fbox{\rule{0pt}{100pt} \rule{450pt}{0pt}} \\
    % \includegraphics[width=\linewidth]{figs/pipeline.pdf}
    % \vspace{-6mm}
    \caption{\textbf{Visualizations per task.}}    
\label{fig:vis-mid}
\end{figure*}

==> figs/teaser.tex <==
\begin{figure*}[ht!]
    \centering
    % \fbox{\rule{0pt}{100pt} \rule{400pt}{0pt}} \\
    \includegraphics[width=\linewidth]{figs/source/main.pdf}
    % \vspace{-6mm}
    \caption{\textbf{Are we making progress in learning mid-level vision representations?}
    High-level visual recognition tasks \textbf{(a)} are the de facto standard for evaluating self-supervised learning methods (SSLs), while evaluations in mid-level vision tasks \textbf{(b)} have largely been ignored in the literature.
    \textbf{(c)} Our analysis reveals that the performance correlation between mid-level and high-level vision tasks is weaker than within high-level tasks alone.
    \textbf{(d)} While SSLs with stronger high-level vision capabilities generally perform better on mid-level vision tasks, several interesting outliers emerge.
    }    
\label{fig:teaser}
\end{figure*}


==> table/evaluation_protocal.tex <==
% \begin{table}[]
% \centering
%  \setlength{\tabcolsep}{4pt}
% % \scriptsize  % Use scriptsize for even more compact layout
% \small
% \begin{tabular}{lllp{2cm}}  % Flexible column widths
% \toprule
% \textbf{Tasks} & \textbf{Dataset} & \textbf{Loss function} & \textbf{Metric} \\
% \midrule
% \rowcolor[gray]{0.9} \emph{\textbf{2D Grouping}}: & & & \\
% \multirow{2}{*}{Segmentation} & VOC07 & \multirow{2}{*}{xxx} & \multirow{2}{*}{AP} \\
%  & VOC12 & & \\
% \midrule
% \rowcolor[gray]{0.9} \emph{\textbf{3D Geometry}}: & & & \\
% \multirow{2}{*}{Depth} & NAVI & \multirow{2}{*}{AdaBin} & \multirow{2}{*}{AbsRel} \\
%  & NYU & & \\
% \arrayrulecolor{gray}\midrule
% \multirow{3}{*}{Surface Normal} & NAVI & \multirow{3}{*}{Angular [xxx]} & \multirow{3}{*}{Mean, Median} \\
%  & NYU & & \\
%  & Taskonomy & & \\
% \arrayrulecolor{gray}\midrule
% \multirow{2}{*}{Curvature} & \multirow{2}{*}{Taskonomy} & L1 & \multirow{2}{*}{Mean Curv.} \\
%  & & L1 + SSIM & \\
% \arrayrulecolor{gray}\midrule
% \multirow{2}{*}{Reshading} & \multirow{2}{*}{Taskonomy} & L1 & \multirow{2}{*}{SSIM} \\
%  & & L1 + SSIM & \\
% \arrayrulecolor{black}  % Reset array rule color to black
% \midrule
% \rowcolor[gray]{0.9} \emph{\textbf{Correspondence}}: & & & \\
% \multirow{3}{*}{Geometric Corr.} & NAVI & \multirow{3}{*}{--} & \multirow{3}{*}{Accuracy} \\
%  & ScanNet & & \\
%  & SPair-71k & & \\
% Image Retrieval & NIGHTS & -- & Retrieval Score \\
% \bottomrule
% \end{tabular}
% \caption{Evaluation protocol for mid-level vision tasks.}
% \end{table}


\begin{table*}[ht!]
\centering
 \setlength{\tabcolsep}{4pt}
% \scriptsize  % Use scriptsize for even more compact layout
\small
\begin{tabular}{lllp{2cm}}  % Flexible column widths
\toprule
\textbf{Tasks} & \textbf{Dataset} & \textbf{Loss function} & \textbf{Metric} \\
\midrule
\rowcolor[gray]{0.9} \emph{\textbf{2D Grouping}}: & & & \\
\multirow{2}{*}{Segmentation} & VOC07 & \multirow{2}{*}{xxx} & \multirow{2}{*}{AP} \\
 & VOC12 & & \\
\midrule
\rowcolor[gray]{0.9} \emph{\textbf{3D Geometry}}: & & & \\
\multirow{2}{*}{Depth} & NAVI & \multirow{2}{*}{AdaBin} & \multirow{2}{*}{AbsRel} \\
 & NYU & & \\
\arrayrulecolor{gray}\midrule
\multirow{3}{*}{Surface Normal} & NAVI & \multirow{3}{*}{Angular [xxx]} & \multirow{3}{*}{Mean, Median} \\
 & NYU & & \\
 & Taskonomy & & \\
\arrayrulecolor{gray}\midrule
\multirow{2}{*}{Curvature} & \multirow{2}{*}{Taskonomy} & L1 & \multirow{2}{*}{Mean Curv.} \\
 & & L1 + SSIM & \\
\arrayrulecolor{gray}\midrule
\multirow{2}{*}{Reshading} & \multirow{2}{*}{Taskonomy} & L1 & \multirow{2}{*}{SSIM} \\
 & & L1 + SSIM & \\
\arrayrulecolor{black}  % Reset array rule color to black
\midrule
\rowcolor[gray]{0.9} \emph{\textbf{Correspondence}}: & & & \\
\multirow{3}{*}{Geometric Corr.} & NAVI & \multirow{3}{*}{--} & \multirow{3}{*}{Accuracy} \\
 & ScanNet & & \\
 & SPair-71k & & \\
Image Retrieval & NIGHTS & -- & Retrieval Score \\
\bottomrule
\end{tabular}
\caption{Evaluation protocol for mid-level vision tasks.}
\end{table*}

==> table/main.tex <==
\begin{figure*}[t!]
    \centering
    \fbox{\rule{0pt}{100pt} \rule{450pt}{0pt}} 
    \caption{Probing self-supervised learning methods in mid-level vision tasks. \zc{We should illustrate the SSLs, the probing methods, and some quick view of key findings here, all comprehensive visualization of mid-level vision tasks.}}
    \label{fig:teaser}
\end{figure*}


==> table/probing_curvature_taskonomy.tex <==
\begin{table*}[th!]
  \newcommand{\rowheader}{\rowcolor{Gray!20}}
  \centering
  \caption{
    \textbf{Curvature Results (Taskonomy Dataset).} Performance metrics for various models on Test Loss, RMS (k1, k2, and avg), and averaged $\delta$ thresholds at 0.1, 0.25, and 0.5.
  }
  \label{tab:taskonomy_curvature}
  \setlength\tabcolsep{5pt}
  \footnotesize
  \begin{tabularx}{\textwidth}{X l c c c c c c c c}
    \toprule
    \textbf{Model} & \textbf{Backbone} & \textbf{Test Loss} & \textbf{RMS$_\mathrm{k1}$} & \textbf{RMS$_\mathrm{k2}$} & \textbf{RMS$_\mathrm{avg}$} & $\boldsymbol{\delta_{0.1, \text{avg}}}$ & $\boldsymbol{\delta_{0.25, \text{avg}}}$ & $\boldsymbol{\delta_{0.5, \text{avg}}}$ \\
    \midrule
    BEiT v2 & ViT-B/16 & 0.4966 & 0.5132 & 0.5034 & 0.5083 & 0.0116 & 0.0355 & 0.3052 \\
    DINO & ViT-B/16 & 0.4979 & 0.5694 & 0.5273 & 0.5483 & 0.0432 & 0.1487 & 0.5150 \\
    Barlow Twins & RN-50 & 0.4956 & 0.5137 & 0.5033 & 0.5085 & 0.0137 & 0.0400 & 0.3036 \\
    BYOL & RN-50 & 0.4959 & 0.5142 & 0.5033 & 0.5087 & 0.0135 & 0.0394 & 0.3027 \\
    ClusterFit & RN-50 & 0.4960 & 0.5143 & 0.5033 & 0.5088 & 0.0134 & 0.0393 & 0.3029 \\
    EVA & ViT-B/16 & 0.4960 & 0.5111 & 0.5033 & 0.5072 & 0.0115 & 0.0351 & 0.3056 \\
    DeepCluster v2 & RN-50 & 0.4957 & 0.5137 & 0.5033 & 0.5085 & 0.0135 & 0.0396 & 0.3028 \\
    DenseCL & RN-50 & 0.4958 & 0.5132 & 0.5033 & 0.5083 & 0.0131 & 0.0385 & 0.3016 \\
    MaskFeat & ViT-B/16 & 0.5097 & 0.5360 & 0.5040 & 0.5200 & 0.0062 & 0.0208 & 0.2765 \\
    Jigsaw & RN-50 & 0.4961 & 0.5133 & 0.5033 & 0.5083 & 0.0127 & 0.0376 & 0.3026 \\
    iBOT & ViT-B/16 & 0.4959 & 0.5135 & 0.5033 & 0.5084 & 0.0132 & 0.0386 & 0.3004 \\
    MILAN & ViT-B/16 & 0.4971 & 0.5132 & 0.5034 & 0.5083 & 0.0111 & 0.0341 & 0.3025 \\
    MoCo v3 & ViT-B/16 & 0.5097 & 0.5360 & 0.5040 & 0.5200 & 0.0062 & 0.0208 & 0.2765 \\
    MoCo v2 & RN-50 & 0.4955 & 0.5133 & 0.5033 & 0.5083 & 0.0139 & 0.0402 & 0.3022 \\
    PixMIM & ViT-B/16 & 0.4956 & 0.5104 & 0.5034 & 0.5069 & 0.0115 & 0.0356 & 0.3059 \\
    PIRL & RN-50 & 0.4958 & 0.5136 & 0.5033 & 0.5084 & 0.0133 & 0.0390 & 0.3037 \\
    RotNet & RN-50 & 0.4965 & 0.5141 & 0.5034 & 0.5087 & 0.0127 & 0.0374 & 0.3009 \\
    SimSiam & RN-50 & 0.4960 & 0.5147 & 0.5033 & 0.5090 & 0.0137 & 0.0397 & 0.3022 \\
    SimCLR & RN-50 & 0.4961 & 0.5144 & 0.5033 & 0.5088 & 0.0135 & 0.0392 & 0.3020 \\
    SwAV & RN-50 & 0.4957 & 0.5136 & 0.5033 & 0.5084 & 0.0135 & 0.0394 & 0.3025 \\
    NPID++ & RN-50 & 0.4958 & 0.5139 & 0.5034 & 0.5087 & 0.0138 & 0.0402 & 0.3023 \\
    MoCo v3 & RN-50 & 0.4956 & 0.5134 & 0.5033 & 0.5084 & 0.0135 & 0.0398 & 0.3035 \\
    DINO & RN-50 & 0.4960 & 0.5139 & 0.5033 & 0.5086 & 0.0133 & 0.0389 & 0.3031 \\
    \bottomrule
  \end{tabularx}
\end{table*}

==> table/probing_reshading_taskonomy.tex <==
\begin{table*}[th!]
  \newcommand{\rowheader}{\rowcolor{Gray!20}}
  \centering
  \caption{
    \textbf{Reshading Results (Taskonomy Dataset).} Performance metrics for various models on Test Loss, RMS, $\epsilon_1$, $\epsilon_2$, $\epsilon_3$, and AbsRel.
  }
  \label{tab:taskonomy_reshading}
  \setlength\tabcolsep{6pt}
  \footnotesize
  \begin{tabularx}{\linewidth}{Xll ccccc}
    \toprule
    \textbf{Model} & \textbf{Backbone} & \textbf{Test Loss} & \textbf{RMS} & $\boldsymbol{\epsilon_1}$ & $\boldsymbol{\epsilon_2}$ & $\boldsymbol{\epsilon_3}$ & \textbf{AbsRel} \\
    \midrule
    Jigsaw & RN-50 & 0.4575 & 0.5214 & 12.03 & 26.55 & 55.01 & 34.1766 \\
    RotNet & RN-50 & 0.4630 & 0.5265 & 11.52 & 25.58 & 54.24 & 34.1220 \\
    NPID & RN-50 & 0.4364 & 0.4995 & 12.78 & 28.43 & 58.47 & 32.3941 \\
    SeLa v2 & RN-50 & 0.4469 & 0.5094 & 12.30 & 26.90 & 56.59 & 33.7867 \\
    NPID++ & RN-50 & 0.4464 & 0.5086 & 12.11 & 27.12 & 57.05 & 33.0832 \\
    PIRL & RN-50 & 0.4519 & 0.5147 & 12.34 & 26.82 & 55.74 & 33.1434 \\
    ClusterFit & RN-50 & 0.4440 & 0.5068 & 12.39 & 27.29 & 57.15 & 34.4799 \\
    DeepCluster v2 & RN-50 & 0.4481 & 0.5104 & 12.48 & 26.91 & 56.10 & 34.1206 \\
    SwAV & RN-50 & 0.4422 & 0.5049 & 12.52 & 27.34 & 57.40 & 33.7734 \\
    SimCLR & RN-50 & 0.4470 & 0.5097 & 12.26 & 26.97 & 56.61 & 33.7568 \\
    MoCo v2 & RN-50 & 0.4527 & 0.5143 & 12.18 & 26.19 & 55.50 & 34.5706 \\
    SimSiam & RN-50 & 0.4428 & 0.5041 & 12.15 & 27.10 & 57.38 & 34.1046 \\
    BYOL & RN-50 & 0.4452 & 0.5075 & 12.14 & 26.90 & 56.99 & 33.1525 \\
    Barlow Twins & RN-50 & 0.4380 & 0.5005 & 12.54 & 27.85 & 58.34 & 34.0821 \\
    DenseCL & RN-50 & 0.4524 & 0.5145 & 12.33 & 26.65 & 55.62 & 33.1017 \\
    DINO & RN-50 & 0.4443 & 0.5082 & 12.93 & 27.80 & 57.04 & 34.4840 \\
    MoCo v3 & RN-50 & 0.5199 & 0.5043 & 12.04 & 25.71 & 54.26 & 33.5495 \\
    DINO & ViT-B/16 & 0.4574 & 0.5186 & 12.07 & 26.27 & 54.77 & 33.3018 \\
    iBOT & ViT-B/16 & 0.4635 & 0.5238 & 11.94 & 25.71 & 53.54 & 33.5193 \\
    MoCo v3 & ViT-B/16 & 0.4424 & 0.5043 & 12.11 & 27.27 & 57.54 & 32.8377 \\
    MAE & ViT-B/16 & 0.4642 & 0.5345 & 11.09 & 24.89 & 52.33 & 33.5341 \\
    MaskFeat & ViT-B/16 & 0.4645 & 0.5259 & 11.91 & 25.55 & 53.46 & 33.5820 \\
    BEiT v2 & ViT-B/16 & 0.5281 & 0.5281 & 11.65 & 25.35 & 53.16 & 33.2942 \\
    MILAN & ViT-B/16 & 0.4696 & 0.5301 & 11.39 & 25.16 & 52.88 & 32.5335 \\
    EVA & ViT-B/16 & 0.5268 & 0.5268 & 11.99 & 26.16 & 53.64 & 32.4247 \\
    PixMIM & ViT-B/16 & 0.4574 & 0.5212 & 12.61 & 26.95 & 54.69 & 33.1802 \\
    \bottomrule
  \end{tabularx}
\end{table*}
